A Geometric Approach For Pose and Velocity Estimation Using IMU and Inertial/Body-Frame Measurements

This paper addresses accurate pose estimation (position, velocity, and orientation) for a rigid body using a combination of generic inertial-frame and/or body-frame measurements along with an Inertial Measurement Unit (IMU). By embedding the original state space, $\so \times \R^3 \times \R^3$, within the higher-dimensional Lie group $\sefive$, we reformulate the vehicle dynamics and outputs within a structured, geometric framework. In particular, this embedding enables a decoupling of the resulting geometric error dynamics: the translational error dynamics follow a structure similar to the error dynamics of a continuous-time Kalman filter, which allows for a time-varying gain design using the Riccati equation. Under the condition of uniform observability, we establish that the proposed observer design on $\sefive$ guarantees almost global asymptotic stability. We validate the approach in simulations for two practical scenarios: stereo-aided inertial navigation systems (INS) and GPS-aided INS. The proposed method significantly simplifies the design of nonlinear geometric observers for INS, providing a generalized and robust approach to state estimation.

==> Section_SE_5_3.tex <==

\section{Preliminaries}\label{section:Notation_Preliminaries}
We denote by $\mathds{Z}_{>0}$  the set of positive integers, by $\R$ the set of reals, by $\R^n$ the $n$-dimensional
Euclidean space, and by $\sphere^n$ the unit $n$-sphere embedded in
$\R^{n+1}$. We use $\|x\|$ to denote the Euclidean
norm of a vector $x\in\R^n$. \red{The $i$-th element of a vector $x\in\R^{n}$ is denoted by $x_i$}. The $n$-by-$n$ identity and zeros matrices are denoted by $I_n$ and $0_{n\times n}$, respectively. By $\mathrm{blkdiag}(\cdot)$, we denote the
block diagonal matrix. The Special Orthogonal group of order three is denoted
by $\so:= \{A\in\R^{3\times3}: \mathrm{det}(A) = 1; AA^{\top} =A^{\top}A=I_3\}$. The set 
$\liealg:=\{\Omega\in\R^{3\times3}:\Omega=-\Omega^{\top}\}$ denotes the Lie algebra of $\so$. The matrix Lie group $\se$ is defined as $\se:=\{X=\mathcal{T}(R,x)\in \se: R\in \so$ and $x\in\R^{3\times5}\}$, with the map $\mathcal{T}:\so \times \R^{15}\to \R^{8\times8}$ defined as
\begin{equation}
    \mathcal{T}(R,x)=\left[\begin{array}{c:c}
  \begin{matrix}
      R
  \end{matrix} &  x\\
  \hdashline \\  [-1em] 
  0_{5\times 3} & I_{5} \\
\end{array}
\right].
\end{equation}
The set $\mathbf{se}_5(3):=\{U=\mathcal{T}(\Omega,v):\Omega\in\liealg$ $v\in\R^{3\times5}\}$ denotes the Lie algebra associated to $\se$. The Lie bracket 
$[A,B]:=AB-BA$ for matrices 
$A$ and $B$ denotes the commutator of two matrices. The vector of all ones is denoted by $\mathds{1}$. For $x,\ y\in\Rthree$, the map $[.]_{\times}:\Rthree\to\liealg$ is defined such that $[x]_{\times}y=x\times y$ where $\times$ is the vector
 cross-product in $\Rthree$. The Kronecker product between two matrices $A$ and $B$ is denoted by $A
 \otimes B$. The  vectorization operator $\vect:\R^{m \times n}\to\R^{(m+n)}$ , stacks the columns of a matrix $A \in \R^{m \times n}$ into a single column vector in $\R^{(m+n)}$.% We introduce the following important orthogonal projection operator $\Pi:\sphere^2 \to \Rthree$ that will be used throughout the paper: 
 %\begin{equation}
%\Pi_x=I_3-xx^{\top},\quad x\in\sphere^2.
%\end{equation}
%Note that $\Pi_x$ is an orthogonal projection matrix which geometrically projects any vector in $\Rthree$ onto the plan orthogonal to vector $x\in\sphere^2$. In addition, one verifies that $\Pi_xy=0_{3\times1}$ if $x$ and $y$ are collinear.  For simplicity and clarity, the argument of time-dependent signals is omitted unless otherwise required.

\subsection{Nonlinear Observer Design  on $\se$}
An~alternative solution to estimate the full attitude matrix $\hat R$  is to cascade the proposed linear observer with a nonlinear complementary filter on $\so$ such as in \cite{mahony2008nonlinear,berkane2017design}. This allows to obtain smooth rotations for all times. Thanks to the proposed observer being globally exponentially convergent and the almost global input-to-state stability (ISS) property of the nonlinear complementary filters on $\so$ (see \cite{wang2021nonlinear}), it is not difficult to show that the interconnection preserves almost global asymptotic stability of the estimation errors. A similar structure, in inertial-frame coordinates, has been proposed \cite{Wang_TAC_2022} for vision-aided INS.

Let $\hat R$ be the estimated rotation matrix on $\so$ obtained from
\begin{equation}\label{equation:R_estimator}
    \dot{\hat R}=\hat R[\omega]_\times+\Delta_R\hat R,
\end{equation}
where $\Delta_R\in\mathfrak{so}(3)$. We define the inertial-frame estimated state as %$\hat{p}^{\mathcal{I}}=\hat{R}\hat{p}^{\mathcal{B}}$, $\hat{v}^{\mathcal{I}}=\hat{R}\hat{v}^{\mathcal{B}}$, $e_1$, $e_2$, $e_3$.
$\hat{x}^{\mathcal{I}}=(I_5\otimes\hat{R})\hat{x}^{\mathcal{B}}$. In view of \eqref{equation:Riccati_observer_full_state}, the dynamics for $\hat x^\mathcal{I}$ are 
\begin{equation}\label{equation:x_I_estimator}
    \dot{\hat x}^\mathcal{I}=(\bar A\otimes I_5+I_5\otimes\Delta_R)\hat x^\mathcal{I}+B\hat Ra^B+K^{\mathcal{I}} (y^{\mathcal{I}}-C^{\mathcal{I}} \hat x^{\mathcal{I}})
\end{equation}
where $K^{\mathcal{I}}=(I_5\otimes\hat R)K(I_{n_y}\otimes\hat R^\top), y^{\mathcal{I}}=(I_{n_y}\otimes\hat R) y$ and $C^{\mathcal{I}}=(I_{n_y}\otimes\hat R)C(I_5\otimes\hat R^\top)$.

Now, let $z_x:=\begin{bmatrix}
p^{\mathcal{I}}&v^{\mathcal{I}}& e_1 & e_2 &e_3    
  \end{bmatrix}$ and $\hat{z}_x$ its estimates, and define $\hat{X}:=\mathcal{T}(\hat{R},\hat{z}_x)$. The obtained state estimator for the pair $(\hat R,\hat x^I)$ given by \eqref{equation:R_estimator} and \eqref{equation:x_I_estimator} is actually an observer on the matrix Lie group $\se$ and can be written as 
\begin{equation}
    \dot{\hat{X}}=\hat XU+[\hat X,D]+\Delta\hat X
\end{equation}
where the innovation term $\Delta$  and the matrices $D$ and $U$ are written as follows,
\begin{flalign}\label{equation:DELTA}
 \hspace{0.9cm}   D&:=\left[\begin{array}{c:c}
 0_{3\times 3}  & 0_{3\times 5}  \\
  \hdashline \\  [-1em] 
  0_{5\times 3}  & \bar{A}^{\top}\otimes I_3 \\
\end{array}
\right],  U:= \left[\begin{array}{c:c}
\wx & \begin{matrix}
    0 & \accelbfr &0_{1\times 3} 
\end{matrix}\\
  \hdashline \\  [-1em] 
  0_{5\times 3} &0_{5\times 5} 
\end{array}
\right],\nonumber\\
\Delta&:=\left[\begin{array}{c:c}
 \Delta_R \in\so\ & \Delta_z\in\R^{3\times5} \\
  \hdashline \\  [-1em] 
  0_{5\times 3}  & 0_{5\times 3} \\
\end{array}
\right],
\end{flalign}
 In fact, the original systems dynamics are given by
\begin{equation}
    \dot{X}=XU+[ X,D]
\end{equation}
which results in the following geometric autonomous error dynamics
\begin{align}
 \dot{\tilde X}&=[\tilde X,D]-\tilde X\Delta \nonumber\\&=\left[\begin{array}{c:c}
-\tilde R\Delta_R  & \tilde z_x(\bar{A}^{\top}\otimes I_3)-\tilde R \Delta_z \\
  \hdashline \\  [-1em] 
  0_{5\times 3}  & 0_{5\times 5}  \\
\end{array}
\right],
\end{align}
%  \begin{bmatrix}        -\tilde R\Delta_R&|&\tilde TS-\Delta_T\tilde T\\       0&|&0     \end{bmatrix},
where $\tilde X=X\hat X^{-1}$, $\tilde R=R\hat R ^{\top}$ and $\tilde z_x=z_x-\tilde R \hat z_x$. The dynamics of $\tilde X$ are \blue{decoupled} \red{(Sif: Not sure since $\tilde R$ appears in block of z)} which is a feature that allows us to use Riccati gain update for the linear subsystem. A possible choice for $\Delta_R$ is inspired from \cite{wang2021nonlinear} as follows:
\begin{equation}
    \Delta_R=\frac{1}{2}\sum_{i=1}^3\rho_i[\hat e_i\times e_i]_\times,\quad \rho_i>0.
\end{equation}
On the other hand, one can shows that 
\begin{equation}
    \vect(\dot{ \tilde z}_x)=(\bar{A}\otimes I_3)-K^{\mathcal{I}}C^{\mathcal{I}})\vect(\tilde{z}_x),
\end{equation}
which leads to the following dynamic equation:
\begin{equation}\label{equation:dynamic_of_z_x}
    \dot{ \tilde z}_x=\tilde z_x(\bar{A}^{\top}\otimes I_3)-\tilde z_x(C^{\mathcal{I}})^{\top}(K^{\mathcal{I}})^{\top}.
\end{equation}
Let $\tilde{z}_y=z_y-\hat{R}\hat{z}_y$ where $z_y$ is defined such that $y^{\mathcal{I}}=\vect(z_y)$ and $\hat{z}_y$ is its estimate, \eqref{equation:dynamic_of_z_x} yields
\begin{equation}\label{equation:dynamic_of_z_x_with_zy}
    \dot{ \tilde z}_x=\tilde z_x(\bar{A}^{\top}\otimes I_3)-\tilde z_y(K^{\mathcal{I}})^{\top},
\end{equation}
thus, $\Delta_z$ can be taken as:
\begin{equation}
    \Delta_z=\tilde R^{\top}\tilde z_y(K^{\mathcal{I}})^{\top}.
\end{equation} 
%\red{what about $\Delta_z$ ? Define $\tilde x=(I_5\otimes R)vec(\tilde z)$ and identify the dynamics of $\tilde x$ with $\dot{\tilde x}=(A-KC)\tilde x$ with $A,K,C$ used in the original Riccati observer. This will give you $\Delta_z$ function of the errors and it should be possible to express it function of the measurements and estimated state.}
%{\color{red}Needs more detail, please also check the equations, I wrote them quickly.}

==> to_do.tex <==
1- if possible delete \bar{A} and rename \bar{\bar{A}} as \bar{A}.
--->already done
2- 

